NAS evaluation is frustratingly hard

Neural Architecture Search (NAS) is an exciting new field which promises to be as much as a game-changer as Convolutional Neural Networks were in 2012. Despite many great works leading to substantial improvements on a variety of tasks, comparison between different methods is still very much an open issue. While most algorithms are tested on the same datasets, there is no shared experimental protocol followed by all. As such, and due to the under-use of ablation studies, there is a lack of clarity regarding why certain methods are more effective than others. Our first contribution is a benchmark of $8$ NAS methods on $5$ datasets. To overcome the hurdle of comparing methods with different search spaces, we propose using a method's relative improvement over the randomly sampled average architecture, which effectively removes advantages arising from expertly engineered search spaces or training protocols. Surprisingly, we find that many NAS techniques struggle to significantly beat the average architecture baseline. We perform further experiments with the commonly used DARTS search space in order to understand the contribution of each component in the NAS pipeline. These experiments highlight that: (i) the use of tricks in the evaluation protocol has a predominant impact on the reported performance of architectures; (ii) the cell-based search space has a very narrow accuracy range, such that the seed has a considerable impact on architecture rankings; (iii) the hand-designed macro-structure (cells) is more important than the searched micro-structure (operations); and (iv) the depth-gap is a real phenomenon, evidenced by the change in rankings between $8$ and $20$ cell architectures. To conclude, we suggest best practices, that we hope will prove useful for the community and help mitigate current NAS pitfalls. The code used is available at https://github.com/antoyang/NAS-Benchmark.

==> intro.bak.tex <==
As the deep learning revolution helped us move away from hand crafted features \citep{krizhevsky2012imagenet} and reach new heights \citep{He2016_resnet,Szegedy2017_inception}, so does Neural Architecture Search (NAS) hold the promise of freeing us from \textit{hand-crafted architectures}, which requires tedious and expensive tuning for each new task or dataset. Identifying the optimal architecture is indeed a key pillar of any deep Automated Machine Learning (AutoML) pipeline.
Research in the last two years has proceeded at a rapid pace and many search strategies have been proposed, from Reinforcement Learning \citep{ZophLe17_NAS,Pham2018_ENAS}, to Evolutionary Algorithms \citep{Real2017_EvoNAS}, to Gradient-based methods \citep{Liu2019_DARTS}.
Still, it remains unclear which approach and search algorithm is preferable. Typically, methods have been evaluated on accuracy alone, even though accuracy is influenced by many other factors besides the search algorithm. 
Comparison between published search algorithms for NAS is therefore either very difficult (complex training protocols with no code available)% and undocumented hyperparameters)
or simply impossible (different search spaces), as previously pointed out \citep{Li2019_random,Sciuto2019_random,lindauer2019best}. 

As a step towards understanding which methods are more effective, we have collected code for $8$ reasonably fast (search time of less than $4$ days) NAS algorithms, and benchmarked them on $5$ well known CV datasets.
Using a simple metric---the relative improvement over the average architecture of the search space---we find that most NAS methods perform very similarly 
%and often marginally above this baseline.
and rarely substantially above this baseline.
The methods used are DARTS, StacNAS, PDARTS, MANAS, CNAS, NSGANET, ENAS and NAO. The datasets used are CIFAR10, CIFAR100, SPORT8, MIT67 and FLOWERS102.

NAS methods have been typically decomposed into three components \citep{elsken2019neural, Li2019_random}: search space, search strategy and model evaluation strategy. This division is important to keep in mind, as an improvement in any of these elements will lead to a better final performance. 
But is a method with a more (expertly) tuned search space a better \textit{AutoML} algorithm? If the key idea behind NAS is to find the optimal architecture, without human intervention, why are we devoting so much energy to infuse expert knowledge into the pipeline?
Furthermore, the lack of ablation studies in most works makes it harder to pinpoint which components are instrumental to the final performance, which can easily lead to \textit{Hypothesizing After the Results are Known} (HARKing; \citealp{gencogluhark})

Paradoxically, the huge effort invested in finding better search spaces and training protocols, has led to a situation in which \textit{any} randomly sampled architecture performs almost as well as those obtained by the search strategies. 
Our findings suggest that most of the gains in accuracy in recent contributions to NAS have come from manual improvements in the training protocol, not in the search algorithms.

Through a number of additional experiments on the widely used DARTS search space \citep{Liu2019_DARTS}, we will show that: 
\textbf{(a)} how you train (the evaluation protocol) has a much bigger impact than the actual architecture chosen;
\textbf{(b)} there is little variance between different architectures, so much so that
\textbf{(c)} hyperparameters like the number of cells, or the seed itself have a very significant effect on the ranking; and 
\textbf{(d)} the specific operations themselves have less impact on the final accuracy than the hand-designed macro-structure of the network.
Notably, we find that the $200+$ architectures sampled from this search space (available at \gitlink) are all within a range of one percentage point (top-1 accuracy) after a standard full training on CIFAR10.
Finally, we include some observations on how to foster reproducibility and a discussion on how to potentially avoid some of the encountered pitfalls. 



==> intro_old.tex <==
%\Red{Why is this work important? Make a list of all methods recently developed for NAS using the DARTS search space or similar. Lots of people are using lots of resources for NAS, so it's important to highlight that there are issues which must be addressed if we don't want to kill dear trees for no reason. Mention papers talking about evaluation of NAS methods + Bench101}

Following the success of the first Neural Architecture Search (NAS) methods in automatically designing neural networks \citep{ZophLe17_NAS,Real2017_EvoNAS}, this subfield of AutoML has received substantial attention.
The problem can be posed as follows: ``given a supervised learning task and a corresponding dataset, which neural network architecture gives the lowest generalisation error?''
NAS proceeds by defining a search space and a search strategy in that space, both of these components being determined a priori.
Many search strategies have been proposed for NAS---Reinforcement Learning, Evolutionary Algorithms, Gradient-based method---though it remains unclear which approach and search algorithm is preferable. Typically, the focus has been on accuracy alone, even though accuracy is determined by many other factors besides the search algorithm. \Red{[.] merge these paragraphs}

Comparison between published search algorithms for NAS is either very difficult (incomplete experimental results, unreleased code, hidden performance-enhancing training protocols, undocumented hyperparameters) or simply impossible (different search spaces), as previously pointed out \citep{Li2019_random,Sciuto2019_random}.
Even when possible, training neural networks remains a computationally very expensive process and therefore consistent comparative results are non trivial to obtain.

%%%%%%%%%%%%%%%%%%%%%
NAS methods have been typically decomposed into three components \citep{elsken2019neural, Li2019_random}: search space, search strategy and model evaluation strategy. This division is important to keep in mind, as an improvement on any of these three components will lead to a better final performance. 
But is a method with a more (expertly) tuned search space a better \textit{AutoML} algorithm? If the key idea behind NAS is to find the optimal architecture, without human intervention, why are we devolving so much energy to infuse expert knowledge into the pipeline?
Furthermore, the lack of ablation studies in most works, makes it harder to pinpoint which components are instrumental to the final performance, and can easily lead to HARKing \citep{gencogluhark}. \Red{[.]}

What we will show in this paper is that so much care was devolved into finding the optimal search spaces and training protocols, that any given randomly sampled architecture performs almost as well as those obtained by the search strategies. We will then explore one of the most commonly used search spaces, \cite{Liu2019_DARTS}, to better understand its properties. Finally, we include some observations on NAS and reproducible and a discussion on how to potentially avoid some of the encountered pitfalls. 

%%%%%%%%%%%%%%%%%%%%%
NAS-Bench-101 \citep{Ying2019_NAS-Bench-101} did the effort to evaluate all $423,000$ architectures of a given search space and proposes a promising framework to evaluate NAS methods, provided that they are implemented in this search space. However, their protocol is not compatible with weight-sharing based methods, as it involves training neural networks seen during the search for multiple epochs. That is a substantial, if necessary, limitation, as most recent methods %that have released their code online 
rely on this hypothesis.

Additionally, two other essential evaluation metrics have been overlooked: (1) the trade-off between computational cost and accuracy; (2) the improvement over a random baseline. 

Our main contributions are :

\begin{itemize}
\item[] %CONTRIBUTIONS:
    \item
    \textbf{Comparison of $8$ methods to random sampling. }
    We provide a sober evaluation of $8$ NAS methods 
    (DARTS, StacNAS, PDARTS, MANAS, CNAS, NSGANET, NAO, ENAS) 
    using publicly available code. We notably report results averaged over multiple runs, and random architectures results in the different search spaces and using the different evaluation protocols.
    %\textbf{Random Search.}
    %We provide a sober evaluation of NAS algorithms with appropriate baselines, putting in perspective the achievements in the field ($\text{NAS}=\text{RS}+\epsilon$, with $\epsilon \to 0$ as $\text{GPU}_{\text{NAS}}/\text{GPU}_{\text{RS}} \to 1$).
    %We conduct an extensive benchmark analysis using 8 recent methods with publicly available source code.
    \item
    \textbf{New datasets.}
    Virtually all NAS works for Image Classification searches on CIFAR10, and eventually transfer their architecture for evaluation on other datasets, notably ImageNet. A limited number also search for architectures on ImageNet \citep{Cai2018_proxylessNAS, MANAS2019}. 
    (REF methods that use any other image datasets)
    It is therefore unclear if NAS methods generalise well to other datasets, without which these methods are incomplete. It is conceivable that some degree of over-fitting occurs.
    This hasn't yet been evaluated. We evaluate the $8$ methods on $5$ datasets (CIFAR10, CIFAR100, SPORT8, MIT67, FLOWERS102).
    \item
    \textbf{Tricks.}
    Common NAS methods are composed of $2$ stages : a search and a a final training that gives an evaluation of the neural network that the algorithm found. The current trend is to add an array of techniques (also known as \textit{tricks}) to this second stage in order to boost accuracy. Accuracy is of course desirable but at the same time this approach masks the quality of the search algorithms and makes it impossible to compare them fairly. Without ablation studies (sensitivity analysis) it remains unclear which search algorithm performs better.
    Our results suggest that most of the gains in accuracy in recent contributions to NAS have come from manual improvements in the training protocol, not in the search algorithms: this clearly conflicts with the goal of AutoML.
    \item
    \textbf{Search Space.}
    Cell-based search spaces, first introduced by \citep{Zoph2018_Cell} enables to search on proxy networks and therefore speed up the search protocol. We provide a deep study of such a search space introduced by \citep{Liu2019_DARTS} that has been reused in many works. We notably found out that the $200$ architectures we sampled from this search space all are within a range of one accuracy percent point after a standard full training on CIFAR10.
    \item
    \textbf{Hyperparameters and Seeds.}
    During both search and evaluation, NAS methods require a number of hyperparameters which need to be tuned for each task/dataset, and add an additional layers of optimisation to the NAS pipeline. However, the cost of tuning these hyperparameters is never reported. Approaches like BOHB can...
    We also show that the variability due to the random seed of the evaluation is not insignificant (at least compared to the improvements typically reported; in the order of $0.15$ p.p.). As such, random seeds are as important as other hyperparameters and should be thought of as a component of the architecture search process.
      
\end{itemize}






